Beyond Accuracy: On the Effects of Fine-tuning Towards Vision-Language Model's Prediction Rationality

Vision-Language Models (VLMs), such as CLIP, have already seen widespread applications. Researchers actively engage in further fine-tuning VLMs in safety-critical domains. In these domains, prediction rationality is crucial: the prediction should be correct and based on valid evidence. Yet, for VLMs, the impact of fine-tuning on prediction rationality is seldomly investigated. To study this problem, we proposed two new metrics called Prediction Trustworthiness and Inference Reliability. We conducted extensive experiments on various settings and observed some interesting phenomena. On the one hand, we found that the well-adopted fine-tuning methods led to more correct predictions based on invalid evidence. This potentially undermines the trustworthiness of correct predictions from fine-tuned VLMs. On the other hand, having identified valid evidence of target objects, fine-tuned VLMs were more likely to make correct predictions. Moreover, the findings are also consistent under distributional shifts and across various experimental settings. We hope our research offer fresh insights to VLM fine-tuning.

==> sec/0_abstract.tex <==
\begin{abstract}
% \small
\normalsize
Vision-Language Models (VLMs), such as CLIP, have already seen widespread applications.
% Researchers are actively engaged in further fine-tuning VLMs in safety-critical domains, where qualified prediction rationality is considered to be crucial:~\textit{the prediction should be correct and based on valid evidence}.
Researchers actively engage in further fine-tuning VLMs in safety-critical domains. 
In these domains, prediction rationality is crucial: \textit{the prediction should be correct and based on valid evidence}.
Yet, for VLMs, the impact of fine-tuning on prediction rationality is seldomly investigated. 
To study this problem, we proposed two new metrics called \textit{Prediction Trustworthiness} and \textit{Inference Reliability}.
We conducted extensive experiments on various settings and observed some interesting phenomena.
% On the one hand, we surprisingly observe the drawback of several mainstream fine-tuning methods.
On the one hand, we found that the well-adopted fine-tuning methods led to more correct predictions based on invalid evidence.
This potentially undermines the trustworthiness of correct predictions from fine-tuned VLMs.
% On the other hand, there are also certain advantages.
% The correct explanations can help enhance predictions made by fine-tuned VLMs.
On the other hand, having identified valid evidence of target objects, fine-tuned VLMs were more likely to make correct predictions.
Moreover, the findings are also consistent under distributional shifts and across various experimental settings.
We hope our research offer fresh insights to VLM fine-tuning.
Our code is available at: https://github.com/deep-real/vlm-pred-rationality. 
% We will release the source code upon acceptance.
% Our source code, and pretrained weights:
\end{abstract}
% \begin{links}
%     \link{Code}{https://github.com/deep-real/vlm-pred-rationality}
%     \link{Extended version}{https://arxiv.org/pdf/2412.13333}
% \end{links}

==> sec/1_introduction.tex <==
\section{Introduction}
\label{sec:intro}

Vision-Language Models (VLMs), such as CLIP~\cite{clip}, have recently begun to see widespread adoption in high-stakes applications, such as healthcare~\cite{medclip} and autonomous driving~\cite{clip2scene}.
A common practice in utilizing VLMs involves undertaking further fine-tuning~\cite{flyp, wise_ft, medclip} in these models to their specific tasks rather than training deep models from scratch.
% However, existing works~\cite{kumar2022calibrated, wortsman2022robust, flyp} that evaluate mainstream fine-tuning methods for VLMs are limited to prediction performances.
While existing studies have evaluated mainstream fine-tuning methods, they have primarily focused on prediction accuracy~\cite{kumar2022calibrated, wortsman2022robust, flyp}, overlooking an essential aspect: \textit{prediction rationality}, where model predictions should not only be accurate but also grounded in valid evidence.
Besides, the current academic community widely accepts that ``clearly explaining a rationale for a classification decision to an end-user can be as important as the decision itself.''~\cite{hendricks2016generating}
One significant reason is that neglecting the model's prediction rationality will cause severe consequences in safety-critical domains.
For example, doctors employ a fine-tuned VLM which can accurately predict the presence of cancer tumors from X-ray images, to help decision-making.
If its predictions are based on erroneous reasons: the input's background instead of tumor region, doctors will lack trust in fine-tuned VLM, leading them to disregard the usage of the model. 
% However, existing works~\cite{kumar2022calibrated, wortsman2022robust, flyp} that evaluate mainstream fine-tuning methods for VLMs ignore the aspect of prediction rationality, limited to prediction accuracies.
Therefore, in this paper, we study a crucial yet seldom investigated question: \textit{how do mainstream fine-tuning methods affect the rationality of VLM predictions?}

% \hspace{1em}
% we first evaluate whether the model focuses on valid evidence when making predictions, using the ``Relevant Mass Accuracy (RMA)'' score~\cite{es_eval1, es_eval2}. 
% To further investigate the effects of fine-tuning for the prediction rationality of VLMs, based on prediction accuracy and RMA score, 
To systematically study this question, we propose two new metrics to evaluate the rationality of VLM predictions after fine-tuning: 
(1) Prediction Trustworthiness (PT): the ratio of correct predictions with valid evidence overall correct predictions. 
(2) Inference Reliability (IR): the percentage of correct predictions given that the model has identified valid evidence of target objects. 
% measure how many correct predictions given that the models have identified valid evidence of target objects.
To assess whether the model focuses on valid evidence for the image classification task, we measure if the generated explanation heatmap from VLMs focuses on the target objects, based on the ``Relevant Mass Accuracy (RMA)'' score~\cite{es_eval2}.
We study the mainstream methods including ``Zero-Shot'' (ZS), ``Linear-Probing'' (LP), ``Finetune Like CLIP Pretrain'' (FLCP), and standard ``Fine-tuning'' (FT). 
We conducted extensive experiments and have obtained novel and consistent findings.
Our results reveal that widely used fine-tuning methods exhibit significant limitations, yet they also possess certain advantages.
Our key findings are summarized as follows:

% \hspace{1em}
\textbf{Will mainstream fine-tuning methods hurt the rationality of VLM predictions? Surprisingly yes!}
% First, we find mainstream fine-tuning methods mostly lead VLMs to give invalid evidence when making predictions.
% For example, with the CLIP-ViT-B/16 model, compared with ZS, the RMA scores of LP (``Linear Probing''), FLCP (``Finetune Like CLIP Pretrain''), and FT (standard ``Fine-tuning'') drop $4.39\%$, $14.98\%$ and $7.28\%$ respectively, despite improving prediction accuracy by $13.53\%$, $20.09\%$ and $20.95\%$, on Stanford-Dogs~\cite{standog} dataset.
With our proposed ``Prediction Trustworthiness'' metric, fine-tuning results in more appearance of samples with correct predictions based on invalid evidence than zero-shot, making the correct predictions untrustworthy. 
% For instance, with the ALBEF-ViT-B/16 model, compared with ZS, the PT scores of LP(``Linear Probing''), FLCP(``Finetune Like CLIP Pretrain''), and FT(standard ``Fine-tuning'') drop $17.2\%$, $13.85\%$ and $27.31\%$ respectively, on CalTech-101~\cite{caltect101} dataset, despite improving prediction accuracies.
For instance, with the ALBEF-ViT-B/16 model, compared with ZS, the PT scores of LP, FLCP, and FT drop $17.2\%$, $13.85\%$ and $27.31\%$ respectively, on CalTech-101~\cite{caltect101} dataset, despite improving prediction accuracies.
And with the CLIP-ViT-B/16 model, compared with ZS, the PT scores of LP, FLCP, and FT drop $6.4\%$, $5.65\%$, and $4.07\%$ respectively, on ImageNet-1K~\cite{imagenet} dataset.
% Notably, our findings concerning prediction rationality diverge from existing works such as~\cite{flyp}, which asserts the superiority of FLCP in prediction performance. 
% This discrepancy underscores the importance of considering different possibilities when evaluating prediction rationality.
Notably, existing work~\cite{flyp} highlights the effectiveness of fine-tuning for VLMs, asserting that FLCP consistently improves prediction accuracy and should be considered the ``standard'' method for fine-tuning CLIP. 
However, our findings suggest that this conclusion does not hold when evaluating the rationality of VLM predictions.
This discrepancy underscores the importance of considering different possibilities when evaluating prediction rationality.

% \hspace{1em}
\textbf{Will valid evidence help enhance predictions made by fine-tuned VLMs? Yes.}
Using our ``Inference Reliability'' metric, we find that when VLMs focus on valid evidence of target objects, the prediction accuracy of fine-tuned VLMs improves.
% compared with zero-shot VLMs.
For example, in the ImageNet-1K dataset, with the CLIP-ViT-B/16 model, LP, FLCP, and FT outperform ZS in IR scores by $12.6\%$, $8.67\%$, and $16.92\%$ respectively.
Existing works~\cite{kumar2022calibrated, wortsman2022robust, flyp}, which study the positive impacts of VLM fine-tuning, are limited to the prediction accuracies. 
Our research provides insights into the impact of fine-tuning VLMs from a novel perspective, highlighting the benefits of fine-tuning in terms of enhancing prediction rationality.

% \hspace{1em}
\textbf{Will out-of-distribution data change our observations? No.}
There is a critical need to make sure that models work reliably in real-world situations, where the data distribution they encounter might be different from what they were trained on.
For instance, the model must maintain stability and effectiveness in autonomous driving applications across various weather conditions.
In parallel, previous work~\cite{clip} has demonstrated the remarkable predictive performance of CLIP in both in-distribution and out-of-distribution data. 
Therefore, we discuss how our observations might change in the context of out-of-distribution data.
% We find that our discoveries remain unaffected with testing distributional shifts.
We find that all our findings remain consistent across various types and magnitudes of distributional shifts, as demonstrated through experiments in ImageNet-C~\cite{imagenet-c}.
% We apply our findings to the scenario which displays the distribution difference between fine-tuning and testing data, manifesting the broad applicability of our discoveries.

% \hspace{1em}
Lastly, we conducted ablation studies to verify the consistency of our findings, which remain consistent across various experimental settings, including different training optimizers, learning rates, explanation heatmap methods, and fine-tuning techniques such as prompt tuning~\cite{coop} and adapter tuning~\cite{tipa}.
% , and ensemble tuning~\cite{cafo}.

% \hspace{1em}
Our contribution lies in discovering new findings through extensive experiments across various benchmarks including ImageNet~\cite{imagenet}, which are typical and widely used in the community.
We provide novel insights about both the strengths and weaknesses of widely adopted fine-tuning strategies for VLMs, from the perspective of the rationality of VLM predictions.
Moreover, our findings remain consistent across evaluation scenarios involving both in-distribution data and out-of-distribution data, as well as under various experimental settings.
This paper provides new insights for people to rethink the effects of mainstream fine-tuning methods for VLMs.

==> sec/2_3_4.1_experimental_setup.tex <==
\section{Preliminaries}

% \subsection{Existing Evaluation Metrics}

% \textbf{Prediction Evaluation.} 
% We first evaluate both VLM predictions and explanations using well-adopted evaluation metrics.
There has been a surge of people exploring VLMs for their downstream tasks.
% A typical way is to use them for image classification~\cite{flyp, bioclip, clipath}.
A typical way is to use them for image classification~\cite{flyp}.
In our prediction evaluations, we study the image classification task and measure model performances using the top-1 accuracy metric.

\hspace{1em}
% \textbf{Explanation Evaluation.} 
% When assessing the correctness of explanations, the criterion is that model's prediction should focus on the valid explanation.
We evaluate whether the model provides valid evidence for its predictions by examining whether the explanation heatmap generated by VLMs focuses on the target objects. 
Specifically, a heatmap that strongly highlights key object regions while showing minimal responsiveness to background pixels indicates valid evidence.
Therefore, we rely on the ``Relevant Mass Accuracy (RMA)'' score~\cite{es_eval1, es_eval2}, which satisfies this criterion by measuring how much ``mass'' one method assigns to pixels within the region of target objects (ground truth).
% Specifically, given the generated explanation heatmap $(H)$ and the ground truth explanation mask $(M)$, the relevance mass accuracy is calculated by determining the ratio of the total heatmap pixel values within the ground truth mask to the sum of all pixel values across the entire heatmap.
% The RMA score is defined as:
% \begin{equation}
%     \text{RMA}(H, M) = \frac{\sum_{p \in M} H_p}{\sum_{p \in M} H_p + \sum_{p \notin M} H_p},
% \label{es_eval}
% \end{equation}
% where $H_p$ represents the value of the heatmap at the position of pixel $p$.
RMA score is calculated by determining the ratio of the total heatmap pixel values within the target object regions, to the sum of all pixel values across the entire heatmap.
It requires both the generated explanation heatmap $(H)$ from VLMs and the ground truth explanation mask $(M)$, whose pixels on the target objects are marked as 1 otherwise marked as 0.
RMA score is defined as:
\begin{equation}
    \text{RMA}(H, M) = \frac{\sum H \odot M}{\sum H},
\label{es_eval}
\end{equation}
where $\odot$ represents Hadamard product.
% It's important to note that evaluation with ground-truth mask follows existing works. 
Note that the evaluations from many studies~\cite{grad-cam, es_eval1} require the presence of ground-truth mask for heatmap localization.
% And RMA is fully calculated with pixel values of explanation heatmap $(H)$.
% The ground-truth mask just indicates whether pixels belong to target objects or backgrounds.

\begin{figure}[t]
  \centering
  \includegraphics[width=0.46\textwidth]{figs/rma_6.pdf}
  \caption{Both (a) and (b) have low responses to the background while (a) pays more attention to the whole body of the bird and (b) pays more attention to the discriminative feature of the bird (head). Compared with the IoU score between (a) and (b), the difference between them is negligible. Moreover, both achieve correct predictions. Input is from CUB-200-2011~\cite{cub} dataset. ``GT'' denotes abbreviation of ``Ground Truth'' and  ``Explan'' denotes abbreviation of ``Explanation''.}
  \label{rma_reliability}
\end{figure}

% \textbf{RMA Reliability.} 
% There exists other metric~\cite{grad-cam} that use the ``Intersection over Union (IoU)'' to evaluate the evidence that prediction bases on.
% IoU relies on the overlapping regions between the explanation heatmap and the ground truth explanation mask.
% However, we argue that the RMA metric provides a more reasonable evaluation for the classification task.
% Existing work~\cite{grad-cam} uses ``Intersection over Union (IoU)'' to evaluate the validity of evidence which supports model predictions.
% It relies on the overlap between the explanation heatmap and the ground truth mask. 
% However, we argue that the RMA metric offers a more reasonable evaluation for classification tasks.
% In Figure~\ref{rma_reliability}, we show two explanation heatmaps, (a) and (b), that are from different models.
% Even though IoU metric treat them differently, both of them achieve correct predictions with valid evidence.
% They both exhibit a low response to background pixels.
% (a) pays attention to the whole body of the bird.
% (b) is also reasonable because it effectively identifies the distinguishing features of the bird, despite not highlighting the more complete bird region as in (a). 
% % This means that under RMA evaluation, we find that different models provide different evidence for their predictions but both of the evidence that prediction bases on are valid.
% This indicates that under RMA evaluation, different models provide distinct evidence for their predictions, yet both sets of evidence are valid.

\hspace{1em}
We emphasize that the RMA metric provides a more reasonable evaluation for classification tasks compared to metrics like ``Intersection over Union (IoU)" used in other works. 
For instance, Grad-CAM~\cite{grad-cam} relies on the IoU score to measure the overlap between the explanation heatmap and the ground truth mask. 
However, the IoU score fails to reasonably evaluate two vastly different yet valid pieces of evidence.
In Figure~\ref{rma_reliability}, we show two explanation heatmaps, (a) and (b), that are from different models.
Even though the IoU metric treats them differently, both of them achieve correct predictions with valid evidence.
They both exhibit a low response to background pixels.
(a) pays attention to the whole body of the bird.
(b) is also reasonable because it effectively identifies the distinguishing features of the bird, despite not highlighting the more complete bird region as in (a). 
This indicates that compared to IoU, RMA evaluation can fairly treat two distinct but valid evidence.

\hspace{1em}
\textbf{Explanation Heatmap Generation.} 
The method we use is directly from ``Generic Attention Attribution''~\cite{chefer2021transformer_mm}.
In this case, the heatmaps are generated from attention maps of the transformer-based model, which is one of the most well-adopted methods, used in recent works including~\cite{rationale_2023_CVPR}. 
It has been demonstrated in existing work~\cite{liu2022rethinking} that it achieves the best faithfulness performance among all well-known explanation methods when applied to transformer-based models.
The main idea is Hadamard's product between attention maps and their gradient to the output.
% The generated explanation heatmaps in each attention layer is defined as:
It is defined as:
\begin{equation}
    \mathbf{\overline{A}} = \mathbb{E}_{h}((\mathbf{\triangledown A} \odot \mathbf{A})^+),
\label{heatmap_formula}
\end{equation}
where $\odot$ is the Hadamard product, $\mathbf{\triangledown A} := \frac{\partial y_t}{\partial \boldsymbol{A}}$ for $y_t$ which is the model’s output for the class $t$ that we wish to visualize.
$\mathbb{E}_{h}$ is the mean across the heads dimension.
The $+$ indicates that the negative contributions are removed before averaging.
Note that the class we explain are based on the index given by the annotations instead of predictions.
% It is also widely employed in many recent works~\cite{rationale_2023_CVPR, Barkan_2023_ICCV}.
% For more details of this heatmap generation method, please refer to~\cite{chefer2021transformer_mm}.

% Lastly, we claim that our used RMA evaluation is reliable and our evaluation is different from existing works about faithfulness evaluations~\cite{rise, faith_1, faith_2}.
% Due to the space limit, please refer to our supplementary materials for more details.

% \textbf{Difference from Faithfulness.}
% We employ the existing explanation generation method~\cite{chefer2021transformer_mm} as a tool to evaluate whether predictions of VLMs are based on valid evidence.
% Our work is different from existing works~\cite{rise, faith_1, faith_2}, which study the correctness of explanation from the perspective of faithfulness; i.e., how accurately an explanation method reflects the true decision-making process of a model. 
% We highlight that faithfulness is beyond the scope of our study due to two reasons.
% (1) Evaluations of faithfulness mainly focus on the assessment of the explanation heatmap generation method correctness. 
% (2) The method we employ has been demonstrated in existing work~\cite{liu2022rethinking} that it achieves the best faithfulness performance among all well-known explanation methods, including ``Rollout''~\cite{rollout} and ``TransAtt''~\cite{chefer2021transformer}, when applied to transformer-based models.
% It is also widely-employed in many recent works~\cite{rationale_2023_CVPR, Barkan_2023_ICCV}.

\section{Our Proposed Evaluations} 
% We argue that existing evaluations cannot be directly used to test the prediction rationality of VLMs: whether model predictions are correct and based on valid evidence.
We present our evaluation protocols with two criteria in mind.
(1) A trustworthy VLM should not produce instances of invalid evidence among samples with correct predictions.
(2) When focusing on the correct predicted objects, a reliable VLM should leverage such valid evidence to achieve correct predictions.
To determine whether the evidence (or rationale) of the model is correct, we use a threshold of 0.5 on the RMA measure. 
Specifically, an RMA score of 0.5 or above is considered valid evidence and vice versa.
As a result, we achieve four scenarios: RR, RW, WR, and WW (Figure~\ref{fig:model-safety}) that are used to formalize our two novel metrics:
% Next, we present the two novel metrics to evaluate the prediction rationality:

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{figs/ModelSafety.pdf}
    \caption{Overview of the four quadrants (RR, RW, WR, WW) of Accuracy and Rationale that are utilized to evaluate prediction rationality.}
    \label{fig:model-safety}
\end{figure}

% Irrational predictions can have hurtful implications for the VLM utility. 
% Suppose there is a VLM used to identify lung lesions in X-rays. 
% It may accurately identify the lesions but it may attribute the existence of disease to unreasonable factors such as shadows, spots, or tears in the X-ray images. 
% This could potentially undermine the doctor's confidence in the model's reliability and limit the board usage of this model.

\hspace{1em}
1. \textbf{Prediction Trustworthiness (PT)}. 
A dependable and trustworthy model should generate valid evidence that corresponds to accurate predictions. 
Hence, we introduce the ``PT'' metric, which calculates the proportion of samples where the prediction is ``right'' and its evidence is also valid or ``right'' (RR) among all samples with right predictions, defined as:
\begin{equation}
    \text{PT} = \frac{{\text{RR}}}{{\text{RR} + \text{RW}}},
\label{formula_pt}
\end{equation}
where ``RW'' denotes data with the ``right'' classifications based on invalid or ``wrong'' evidence.
It is evident that an increase in the number of RW samples, i.e. irrational predictions, results in a decrease in PT scores.

\hspace{1em}
2. \textbf{Inference Reliability (IR)}. 
Given that the model could pinpoint the regions of target objects, a reliable model should make correct predictions.
Consequently, we introduce the ``IR'' metric, which calculates the proportion of samples with correct prediction and valid evidence among all samples with valid evidence of target objects, defined as:
\begin{equation}
    \text{IR} = \frac{{\text{RR}}}{{\text{RR} + \text{WR}}},
\label{formula_ir}
\end{equation}
where ``WR'' denotes data with incorrect classifications with valid evidence.
An increase in the number of WR samples results in a decrease in IR scores.

% To see whether each data sample is provided with valid evidence, we need to convert the continuous RMA values for each sample into binary 0-1 values. 
% We use 0.5 as a natural threshold for each sample.
% We consider samples with RMA higher than this threshold to be ``valid'', otherwise, they are considered ``invalid''.

% Our proposed two metrics are inspired by existing work~\cite{rationale_2023_CVPR}, which requires VLMs to not only provide the correct category for input images but also offer fine-grained language descriptions that explain their predicted category.
% However, in the field of computer vision, there has been very little research about consistency between prediction and explanation from VLMs.
% Moreover, existing works such as~\cite{rationale_2023_CVPR} did not study the effect of mainstream fine-tuning methods on the prediction rationality of VLMs, which is crucial for board applications of VLMs in safety-critical domains.

\section{Experiments}

\subsection{Experimental Setup}
\textbf{Fine-tuning Methods.}
In this paper, we study fundamental methods including: (1) Zero-Shot (ZS), (2) Linear-Probing (LP), (3) Finetune Like CLIP Pretrain (FLCP), and (4) Fine-tuning (FT). 
% Note that ``ZS" is the method before fine-tuning, and ``LP, FLCP, FT" are after fine-tuning. 
For detailed information on these methods, please refer to our supplementary material in the extended version of our paper.
% For detailed information on these methods, please refer to our supplementary material.

% Note that ``ZS" is the method before fine-tuning, and ``LP, FLCP, FT" are after fine-tuning. 

\hspace{1em}
\textbf{Models.} 
We study four VLMs: the first two models are CLIP-ViT-B/32 \& 16~\cite{clip} from OpenAI, which manifest powerful zero-shot performances on image classification. 
% The next two are ALBEF-ViT-B/16~\cite{albef} (pretrained on 14M image-text pairs) and BLIP-ViT-B/16~\cite{blip} (pretrained on 129M image-text pairs) from Salesforce, both of which performances on image classification task are investigated on \cite{satin, omnivl}.
The next two models are ALBEF-ViT-B/16~\cite{albef}, pretrained on 14M image-text pairs, and BLIP-ViT-B/16~\cite{blip}, pretrained on 129M image-text pairs, both developed by Salesforce. Their performances on the image classification task are also investigated in many works~\cite{satin, omnivl}.

\hspace{1em}
\textbf{Fine-tuning Setups.} 
We maintain a consistent batch size and training epoch across all three fine-tuning methods (LP, FLCP, FT) for the same dataset and model. 
We employ the Adam~\cite{adam} optimizer during the fine-tuning. 
For more details about fine-tuning, please consult our supplementary material.

\hspace{1em}
\textbf{Datasets.} 
In this paper, we conduct experiments on several datasets, including ImageNet~\cite{imagenet}, CalTech-101~\cite{caltect101}, Stanford-Dogs~\cite{standog}, CUB-200-2011~\cite{cub}, and ImageNet-C~\cite{imagenet-c}.
In CUB-200-2011 and CalTech-101 datasets, the 0-1 segmentation mask annotations directly serve as ground truth explanation masks.
For images with bounding box annotations surrounding predicted instances (ImageNet, ImageNet-C, Stanford-Dogs), we generate ground truth explanation masks as follows: given initial masks whose pixel values are all zero, we mark the mask areas within boxes as one.
For more detailed information about these datasets, please refer to the supplementary material.

==> sec/4.2_weakness.tex <==
\subsection{Weaknesses of Fine-tuning}
\label{chap_weakness}

\input{tabs/tab_pred}

\input{tabs/tab_pt_ir_2}

% \textit{Question: How do mainstream fine-tuning methods hurt VLM explainability?}
\textit{Question: Will mainstream fine-tuning methods hurt the rationality of VLM predictions?}

% \textit{Answer 1: Surprisingly yes! Mainstream fine-tuning methods mostly lead VLMs to give invalid evidence when making predictions.}

% % We first evaluate with existing prediction and explanation accuracy scores.
% As shown in Table~\ref{tab_what}, when compared with ZS, these current mainstream fine-tuning methods (LP, FLCP, FT) generally exhibit decline in the RMA scores, even though they contribute to enhanced prediction accuracies.
% For example, in the ImageNet-1K dataset with the CLIP-ViT-B/16 model, the RMA scores of LP, FLCP, and FT drop $5.52\%$, $3.66\%$ and $4.74\%$ respectively, in contrast to ZS, although their prediction accuracies improve ZS method by a large margin.
% Based on these experimental results, we infer that fine-tuning makes explanation heatmaps of VLMs more focused on the image pixels which are irrelevant to the predicted object, making it hard to explain the reason for improved accuracies from fine-tuning.

% We observe that compared with the zero-shot (ZS) method, current well-adopted fine-tuning methods (LP, FLCP, and FT) manifest enhanced responses of VLMs in pixels associated with information that is irrelevant to predicted categories.
% For instance, from leftmost third-row comparisons, besides the prediction object, diving mask, fine-tuning methods have more responses to the pixels of water and human feet than ZS.
% For instance, from the leftmost first-row comparisons, fine-tuning makes VLMs enhance responses on the human body or background instead of the hat (predicted category).
% In our visualizations of the Stanford-Dogs dataset, we observe a similar phenomenon, where results from the fifth row show that LP tends to increase the response on human faces.
% By visualizing explanation heatmaps of four studied methods, we further validate our assumptions drawn from the explanation accuracy in Table~\ref{tab_what}: fine-tuning results in explanation heatmaps generated by VLMs becoming more concentrated on image pixels unrelated to the predicted objects.
% We explore the mechanisms by which fine-tuning alters explanation heatmaps.
% We find that resulting in decreased focus on regions of the predicted target objects. 
% Compared with zero-shot, 
\hspace{1em}
\textit{Answer: Surprisingly yes! The well-adopted fine-tuning methods decrease the trustworthiness of VLM predictions in most settings: causing more samples with correct predictions based on invalid evidence.}

% \begin{figure*}[h]
%   \centering
%   \includegraphics[width=1.0\textwidth]{figs/pecm_albef_clip16.pdf}
%   \caption{Experimental results with our proposed PECM. Compared with ZS, the well-adopted fine-tuning methods tend to cause a higher occurrence of RW samples. But they also contribute to more RR and fewer WR samples. The additional impacts caused by these phenomena are further demonstrated in Table~\ref{tab_ptir}. Please check our supplementary materials for results with the CLIP-ViT-B/32 and BLIP-ViT-B/16 models.}
%   \label{fig_rationale}
% \end{figure*}

% As shown in Figure~\ref{fig_rationale}, our findings indicate that fine-tuning methods lead to a higher occurrence of RW samples compared with ZS method, resulting in more instances where predictions are correct but the explanations are inaccurate.
% For example, on the ImageNet-1K dataset with CLIP-ViT-B/16 model, LP, FLCP, and FT result in higher RW ratios by $6.65\%$, $9.2\%$, and $5.63\%$ than ZS, respectively. 
% Similarly, in the CalTech-101 dataset, when compared with ZS using the CLIP-ViT-B/16 model, they lead to higher RW ratios by $10.08\%$, $3.17\%$, and $8.93\%$, respectively.
% We infer this is potentially another reason why mainstream fine-tuning methods lead to worse explanation accuracies for VLMs.
% This indicates the improved predictive accuracy is unrelated to good explainability.

% We further observe that the increase in RW ratios can lead to negative prediction trustworthiness.
% More specifically, fine-tuning tends to decrease the ratio of samples where explanations are correct among all samples with correct predictions.
% As shown in Table~\ref{tab_ptir}, we find mainstream fine-tuning methods lead to worse prediction trustworthiness, even though improving the prediction accuracies (see Table~\ref{tab_pred}).
\hspace{1em}
Although fine-tuning is able to improve the prediction accuracies of VLMs (see Table~\ref{tab_pred}), we find mainstream fine-tuning methods lead to worse prediction trustworthiness, as shown in Table~\ref{tab_ptir}.
For instance, in the ImageNet-1K dataset, with CLIP-ViT-B/16 model, compared with ZS, fine-tuning deteriorates ``Prediction Trustworthiness (PT)'' performances by $6.4\%$, $5.65\%$ and $4.07\%$ respectively.
Our experimental results confirm the significant drawbacks of mainstream fine-tuning methods for VLMs: fine-tuning results in more instances where predictions are correct but the evidence which VLMs base on is invalid.
This results in a reduced level of trustworthiness to VLM predictions.
Lastly, there are rare exceptions with increased PT scores. 
This is likely due to the low zero-shot prediction accuracy of ALBEF (12.43\%) and BLIP (16.88\%) on CUB-200-2011. 
Fine-tuning introduces the missing knowledge to these models, leading to increased PT.
% The results also indicate that compared with the ZS method, fine-tuning results in more instances where predictions are correct but the evidence which VLMs base on is invalid.

\hspace{1em}
% \textbf{Why does fine-tuning decrease the trustworthiness of VLM predictions?}
To further support our observation, we provide visualizations of the explanation heatmaps in Figure~\ref{fig_vis_id}.
% We only show results on the CLIP-ViT-B/32 model with ImageNet-1K datasets due to space constraints.
% Please refer to our supplementary materials for more visualizations.
% We further shown some visualizations of the explanation heatmap in Figure~\ref{fig_vis_id} and 
We observe that widely adopted fine-tuning methods often amplify the responses of VLMs to pixels containing information irrelevant to the predicted objects.
For instance, from the leftmost first-row comparisons, fine-tuning makes VLMs enhance responses on the human body or background instead of the hat (predicted category).
Here we only show results on the CLIP-ViT-B/32 model with ImageNet-1K datasets due to space constraints.
Please refer to our supplementary material for more visualizations.

\hspace{1em}
\textbf{Why does finetuning decrease trustworthiness?}
(1) VLMs tend to exploit the easiest path to minimize loss during finetuning, often picking up on spurious correlations or shortcuts present in the data. 
For instance, if all images of a particular class contain a common watermark or background, VLMs may associate that feature with the class label instead of learning the actual characteristics of the object. 
(2) Standard fine-tuning objectives usually prioritize improving prediction accuracy, but they do not account for the validity of the evidence used. 
As a result, there is no built-in mechanism to guide the model to focus on valid evidence.

\hspace{1em}
In recent years, there have been some discussions regarding the excellence of fine-tuning for VLMs.
For example, existing work~\cite{flyp} shows that FLCP leads to uniformly better prediction performances.
They claim that FLCP should be adopted as the ``standard'' method for fine-tuning CLIP.
However, based on our discoveries, we contend that this conclusion doesn't apply when considering the rationality of VLM predictions. 
Although FLCP significantly enhances VLMs' prediction accuracies, we find that FLCP leads VLMs to provide more invalid evidence when making correct predictions, weakening the prediction trustworthiness of VLMs than ZS.
This disparity highlights the significance of considering different possibilities when evaluating VLMs' prediction rationality.

\begin{figure*}[h]
  \centering
  \includegraphics[width=1.0\textwidth]{figs/vis_id_in_2.pdf}
  \caption{Visualization comparisons among different methods. Compared with zero-shot (ZS), current mainstream fine-tuning methods (LP, FLCP, and FT) for VLMs tend to show enhanced responses in background pixels that are irrelevant to predictions. Here we select the samples for which all four methods make correct predictions. Here we display bounding box annotations indicating the positions of the predicted target.}
  \label{fig_vis_id}
\end{figure*}

==> sec/4.3_strength.tex <==
\subsection{Strengths of Fine-tuning}
\label{chap_strength}

% \textit{Question: How do mainstream fine-tuning methods benefit VLM explainability? }
\textit{Question: Will valid evidence help enhance predictions made by fine-tuned VLMs?}

% \textit{Observation: They tend to exhibit good inference reliability, i.e., given the correct features, the fine-tuned VLMs are more likely to make the predictions correct.}
\hspace{1em}
\textit{Answer: Yes, they exhibit good inference reliability; i.e., when focusing on the valid evidence of target objects, fine-tuned VLMs are more likely to make correct predictions.}
% than zero-shot method.}

\hspace{1em}
This phenomenon indicates better inference reliability of fine-tuning compared with ZS, as shown in Table~\ref{tab_ptir}.
% We observe from Table~\ref{tab_ptir} that fine-tuning for VLMs can significantly enhance the capabilities of inference reliability.
For example, in the ImageNet-1K dataset, with the CLIP-ViT-B/16 model, LP, FLCP, and FT outperform ZS by $12.6\%$, $8.67\%$, and $16.92\%$ respectively; with the CLIP-ViT-B/32 model, LP, FLCP, and FT outperform ZS by $13.82\%$, $10.75\%$, and $18.25\%$ respectively.
This indicates that fine-tuning approaches contribute to less WR than ZS.
When VLMs identify valid evidence for target objects, fine-tuning is more likely to produce correct predictions.

\hspace{1em}
Existing works~\cite{kumar2022calibrated, wortsman2022robust, flyp} are limited to the impact of mainstream VLM fine-tuning methods regarding predictive accuracies, ignoring their positive impacts on VLM prediction rationality. 
In this paper, we have analyzed and explored the benefits of fine-tuning VLMs from a new perspective.
Our experimental results show that fine-tuning has its merits and is not completely worthless for the prediction rationality of VLMs.

\hspace{1em}
In summary, we conducted extensive experiments to validate the existing mainstream VLM fine-tuning methods in terms of both their strengths and weaknesses from a prediction rationality perspective. 
On the one hand, fine-tuning leads to good inference reliability: when provided with valid evidence of target objects, fine-tuned VLMs are more likely to generate accurate predictions.
On the other hand, we also confirm that mainstream fine-tuning methods tend to hurt the inherent capabilities of VLMs, specifically in terms of prediction trustworthiness.
These are aspects that merit attention from the community of machine learning.

==> sec/4.4_ood.tex <==
\subsection{Analysis on Out-of-Distribution Data}
\label{chap_ood}

% \textit{Question: How do data distributional shifts affect the conclusions?}
\textit{Question: Will out-of-distribution data change our observations?}

% \textit{Observation: Yes, the conclusions are consistent with scenarios where the training and testing data distributions are the same.}
% \textit{Takeaway: Our conclusions are robust against distributional shifts. All conclusions are held.}
% \textit{Takeaway: Our conclusions remain robust even in the presence of distributional shifts, with all findings remaining consistent.}
\hspace{1.3em}
\textit{Answer: No, all findings remain consistent.}

\hspace{1em}
Distributional shifts has garnered significant attention in the field of machine learning~\cite{fc_cvpr, fc_iclr}.
During the fine-tuning, the distributional discrepancy between the fine-tuning and testing data is worth considering.
% On the one hand, in real-world applications, the models may encounter varying data distributions, making it crucial to validate the generalization performance of models on data under distributional shifts. 
% On the other hand, 
Real-world data distributions can change due to factors such as time, location, and environment. 
Testing on out-of-distribution data helps simulate these changes, ensuring the model performs well in diverse scenarios. 
For example, in autonomous driving, the models need to remain stable in multiple weather conditions.

\hspace{1em}
In this section, we study the fine-tuning methods when testing on out-of-distribution data. 
Here we use the ImageNet-C dataset, which includes multiple corruption categories and levels of severity. 
As shown in Figure~\ref{fig_ood}, our key findings are as follows:
\begin{enumerate}
    \item Fine-tuning on in-distribution data can enhance the prediction accuracy for out-of-distribution data.
    \item However, the mainstream fine-tuning methods still compromise the prediction trustworthiness of VLM, which brings more samples with correct prediction based on invalid evidence, compared with zero-shot.
    % \item Compared with ZS, fine-tuning tends to bring more RW samples: correct prediction but wrong explanation. This indicates that the improved accuracy from fine-tuning has little correlation with explanation ability.
    \item Fine-tuning tends to enhance the inference reliability of VLMs: when focusing on correct prediction objects, fine-tuned VLMs are more likely to give correct predictions.
\end{enumerate}
Therefore, we extend our previous findings to scenarios involving out-of-distribution data, demonstrating the consistency of our discoveries.

\begin{figure}[h]
  \centering
  \includegraphics[width=0.48\textwidth]{figs/ood_fig_f00.pdf}
  \caption{Experimental results on out-of-distribution data. Our discoveries remain consistent across various types and magnitudes of distributional shifts. The x-axis in all figures represents the strength of corruption, where a strength of 0 indicates the results of different methods on the original ImageNet validation data. Due to space constraints, we only show results with CLIP-ViT-B/32 and four types of corruption in the main paper. For more results, please refer to our supplementary material.}
  \label{fig_ood}
\end{figure}

\hspace{1em}
% We also observe a significant decrease in prediction accuracy as the corruption strength increases. 
% Compared with cases where the distributions of fine-tuning and testing data are identical, we also note a marked decline in prediction accuracy across all methods as the level of data corruption intensifies.
Our conclusions also remain unaffected when the prediction accuracies decrease caused by corruption strength increases. 
Therefore, we think our findings may not change with variations in model prediction accuracy.

==> sec/4.5_ablation_study.tex <==
\subsection{Ablations studies}
To ensure the consistency of our findings across different experimental settings, we perform a comprehensive series of ablation studies.
We investigate the effects under different setups including:
(1) Experiments with another popular optimizer: AdamW~\cite{adamw}.
(2) Experiments with another widely-used explanation method: gradient of attention ($\mathbf{\nabla A}$) based~\cite{grad_att} method.
The main idea of this method is to utilize the gradient of attention to the output as an explanation heatmap, where $\mathbf{\triangledown A} := \frac{\partial y_t}{\partial \boldsymbol{A}}$ for $y_t$ which is the model’s output for the class $t$.
(3) Results with different fine-tuning learning rates (abbreviated as ``LR''): $5e-4$ for ``LP'', $3e-6$ for ``FLCP'', and $2e-5$ for ``FT'', compared with the original setup, where we set learning rates as $1e-3$ for ``LP'', $5e-6$ for ``FLCP'', and $1e-5$ for ``FT''.
For the original learning rate settings regarding other models and datasets please refer to our supplementary material.
Note that the aforementioned three experiments are conducted with the CLIP-ViT-B/32 model on the ImageNet-1K.

% \begin{figure}[h]
% % \vspace{-35pt}
%   \centering
%   \includegraphics[width=0.45\textwidth]{figs/ab_fig_4.pdf}
% \caption{Ablation studies with our proposed PECM.}
% \label{fig_ab}
% % \vspace{-20pt}
% \end{figure}

\hspace{1em}
As shown in Table~\ref{tab_ab}, \textit{our findings remain unaffected} with multiple setups. 
% Specifically, the mainstream fine-tuning methods mostly deteriorate explanation accuracy for VLMs, and cause more samples with correct prediction but wrong explanation, although with improved prediction accuracy. 
% On the other hand, fine-tuning tends to exhibit good inference reliability.
On the one hand, prevalent fine-tuning approaches tend to increase the instances with correct predictions based on invalid evidence, despite the enhancement in prediction accuracy. 
On the other hand, fine-tuning typically demonstrates strong inference reliability.

\hspace{1em}
Recently, there have been other fine-tuning techniques proposed by the community including prompt tuning~\cite{coop}, and adapter tuning~\cite{tipa}.
% , and ensemble tuning~\cite{cafo}. 
We find that \textit{our findings are also consistent under these fine-tuning methods.} 
Due to the space limits please refer to our supplementary material for the related experimental results and introduction of these methods.

==> sec/5_related_work.tex <==
\section{Related Works}
\label{sec:formatting}

%-------------------------------------------------------------------------
% \subsection{Vision-language Foundation Models}
\subsection{Multimodal Foundation Models}

In recent years, there has been a surge of interest in research regarding Vision-Language Models (VLMs). 
% A proliferation of these VLMs, including but not limited to, has emerged in response to this burgeoning field of study.
These VLMs~\cite{clip, albef, blip, flava, align, alignprompt, declip, florence, glip, otter, pali, regionclip, vilt, uniter}, have attracted substantial attention due to their remarkable capacity to achieve robust performance, both in zero-shot and fine-tuned scenarios, across a diverse spectrum of vision-language-related tasks~\cite{vqa, itr, ve, nlvr}.
% These tasks encompass Visual Question Answering (VQA), Image-Text Retrieval (ITR)~\cite{itr}, Visual Entailment (VE)~\cite{ve}, as well as Visual Grounding and Natural Language for Visual Reasoning (NLVR)~\cite{nlvr}, among others.
Notably, CLIP~\cite{clip}, as a prominent exemplar in this domain, has also demonstrated exceptional zero-shot performance in image classification. 
The contrastive learning approach it employs has also found applications in fields such as multiview analysis~\cite{cmc} and egocentric video understanding~\cite{qitong_iccv}.
% Its resilience to distributional shifts surpasses that of conventional ResNet-101~\cite{resnet} models trained on the ImageNet~\cite{imagenet} dataset.
% Recently, researchers have undertaken the fine-tuning of VLMs with a view to tailoring them more effectively to their downstream application domains. 
Recently, researchers have engaged in fine-tuning~\cite{flyp} VLMs to better adapt them to specific downstream tasks.
However, the impact of such training on the prediction rationality of these models remains an open research problem, one that warrants in-depth exploration and investigation.
% In parallel, several ``Multimodal Large Language Models'' (MLLMs) like LLaVA~\cite{llava, lisa, pixellm} have been proposed.
% Following them, parameter-efficient fine-tuning methods for these MLLMs have been proposed or applied, including Visual Instruction Tuning~\cite{llava}, Low-Rank Adaptation (LoRA)~\cite{lora}, and AutoPEFT~\cite{AutoPEFT}.
% The effects of fine-tuning on prediction rationality of MLLMs could be an interesting future work.

\begin{table}[t]
\centering
% \footnotesize
\scriptsize
\begin{tabular}{c|c|cccc}
\hline
\multirow{2}{*}{Setup}                                                                              & \multirow{2}{*}{Evaluations} & \multicolumn{4}{c}{Methods}   \\ \cline{3-6} 
                                                                                                    &                              & ZS    & LP    & FLCP  & FT    \\ \hline
% \multirow{3}{*}{Original}                                                                           & Pred. Acc.(\%) ↑             & 58.41 & 72.21 & 70.81 & \textbf{76.62} \\
%                                                                                                     % & RMA(\%) ↑                    & \textbf{79.40} & 74.22 & 76.62 & 76.14 \\
%                                                                                                     & PT(\%) ↑                     & \textbf{89.39} & 84.05 & 85.48 & 86.29 \\
%                                                                                                     & IR(\%) ↑                     & 61.09 & 74.91 & 71.84 & \textbf{79.34} \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}AdamW \\ Optimizer\end{tabular}}                         & Pred. Acc.(\%) ↑             & 58.41 & 72.22 & 70.88 & \textbf{76.53} \\
                                                                                                    % & RMA(\%) ↑                    & \textbf{79.40} & 74.34 & 76.68 & 76.26 \\
                                                                                                    & PT(\%) ↑                     & \textbf{89.39} & 84.23 & 85.53 & 86.46 \\
                                                                                                    & IR(\%) ↑                     & 61.09 & 74.93 & 71.93 & \textbf{79.26} \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}$\nabla A$ \\ Explanation \\ Heatmap\end{tabular}}       & Pred. Acc.(\%) ↑             & 58.41 & 72.21 & 70.81 & \textbf{76.62} \\
                                                                                                    % & RMA(\%) ↑                    & \textbf{69.11} & 61.46 & 62.49 & 63.05 \\
                                                                                                    & PT(\%) ↑                     & \textbf{74.79} & 63.62 & 65.21 & 65.76 \\
                                                                                                    & IR(\%) ↑                     & 61.18 & 75.18 & 71.87 & \textbf{79.68} \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Different LRs \\ Compared with \\ Original\end{tabular}} & Pred. Acc.(\%) ↑             & 58.41 & 72.28 & 70.05 & \textbf{75.51} \\
                                                                                                    % & RMA(\%) ↑                    & \textbf{79.40} & 74.41 & 77.01 & 76.18 \\
                                                                                                    & PT(\%) ↑                     & \textbf{89.39} & 84.72 & 86.19 & 86.59 \\
                                                                                                    & IR(\%) ↑                     & 61.09 & 74.91 & 71.21 & \textbf{78.62} \\ \hline
\end{tabular}
\caption{
Ablation studies with prediction accuracy, and our proposed ``Prediction Trustworthiness (PT)'' and ``Inference Reliability (IR)'' metrics.
% Ablation studies with prediction accuracy, and our proposed ``PT'' and ``IR'' metrics.
Our findings are unaffected under different experimental setups.
The best score is bolded.}
\label{tab_ab}
% \vspace{-10pt}
\end{table}

%-------------------------------------------------------------------------
\subsection{Explainable Machine Learning}

Explainable Machine Learning (XML) is crucial for promoting transparency, trust, accountability, and fairness in AI systems.
% , as well as for enhancing the usability and acceptance of AI-driven technologies across various industries and applications.
Researchers frequently employ techniques to explain neural network operations and decision-making regarding input data. 
Activation heatmaps such as Grad-CAM~\cite{grad-cam}, visualize important regions for specific classes. 
% Model-agnostic methods, such as LIME~\cite{lime}, explain individual sample predictions, while SHAP~\cite{shap} values assess feature contributions to model predictions. 
In light of the proliferation of transformer-based models~\cite{vit}, researchers start exploring the feasibility of utilizing attention maps, taking it as a way to provide explanations~\cite{chefer2021transformer_mm}.
In order to evaluate the quality of these explanation generation methods, existing works including~\cite{rise} study from the perspective of faithfulness; i.e., how accurately an explanation method reflects the true decision-making process of a model. 
% We highlight that faithfulness is beyond the scope of our study due to two reasons.
% (1) Evaluations of faithfulness mainly focus on the assessment of the explanation heatmap generation method correctness. 
% (2) The method we employ has been demonstrated in existing work~\cite{liu2022rethinking} that it achieves the best faithfulness performance among all well-known explanation methods, including ``Rollout''~\cite{rollout} and ``TransAtt''~\cite{chefer2021transformer}, when applied to transformer-based models.
% It is also widely-employed in many recent works~\cite{rationale_2023_CVPR, Barkan_2023_ICCV}.
% A recent study by Li \textit{et al.}~\cite{dre} undertakes a comprehensive examination of the robustness of data-driven explanations when subjected to naturally occurring distributional shifts. 
% This investigation reveals that even when deep learning models make correct predictions, their associated explanations remain unreliable when confronted with out-of-distribution data.
% In parallel, Mao \textit{et al.}~\cite{rationale_2023_CVPR} propose the concept of a reliable model, emphasizing the importance of the "doubly-right" criterion: both accurate predictions and coherent explanations.
In parallel, Mao et al.~\cite{rationale_2023_CVPR} propose the concept of a reliable model, emphasizing the importance of the "doubly-right" criterion: both accurate predictions and fine-grained language explanations of model decision-making.
% This criterion dictates that a reliable model not only yields accurate predictions but also furnishes explanations that are conceptually sound and reasonable.
% More specifically, this criterion requires that a reliable model not only yields accurate predictions but also provides fine-grained language descriptions to explain its decision-making.
Recently, some works~\cite{tang_nips, tang_eccv} have increasingly required VLM models to deliver not only accurate predictions but also correct rationales.
In this paper, we explore the impact of widely accepted fine-tuning methods on the prediction rationality of VLMs for vision tasks such as image classification, providing novel insights about VLM fine-tuning within the XML research community.
And we highlight that faithfulness is beyond the scope of our study due to two reasons.
On the one hand, faithfulness evaluations primarily focus on assessing the correctness of heatmap explanation methods.
On the other hand, existing work~\cite{liu2022rethinking} verified the superiority of our employed explanation generation method.

==> sec/6_conclusion.tex <==
\section{Conclusion}

Prediction rationality is an important aspect to consider when fine-tuning Vision-Language Models (VLMs), especially in high-stakes applications. 
This paper provides a comprehensive assessment of the commonly used fine-tuning approaches, presenting some insights on both advantages and disadvantages.
% : positive inference reliability but poor prediction trustworthiness.
% Moreover, other drawbacks of these methods are revealed: compared with ZS, they lead to a decrease in explanation accuracy and tend to cause spurious correlations between predictions and explanations.
On the one hand, they generally demonstrate strong inference reliability.
More specifically, when focusing on the valid evidence of target objects, the fine-tuned VLMs are more likely to make correct predictions.
On the other hand, fine-tuning often results in undermining the trustworthiness of VLM predictions by bringing more data samples with correct predictions based on invalid evidence.
% We further extended our study to scenarios involving testing data with distribution shifts, where our previous conclusions still hold.
We further observe that our discoveries are consistent across various types and magnitudes of distributional shifts, and remain unaffected with multiple setups.
To ensure that VLMs can be reliably used in high-stack applications, it will be crucial to study new fine-tuning methods that can improve VLM prediction rationality. 
% It is also interesting to study the effect of fine-tuning on the prediction rationality of MLLMs.
We leave it as future works.
We expect our research may provide useful experience and advance the study of VLM fine-tuning.
% We expect our research may advance the study of VLM fine-tuning.

\section{Acknowledgements}
This work is supported by the NSF CAREER Award No. 2340074, the NSF SLES Award No. 2416937, the NSF III CORE Award No. 2412675, and the DoD DEPSCoR Award AFOSR FA9550-23-1-0494. 
Any opinions, findings and conclusions or recommendations expressed in this material are those of the authors and do not reflect the views of the supporting entities.

==> sec/checklist.tex <==
% \clearpage
% \setcounter{page}{1}
% \maketitlesupplementary

% \renewcommand\thesection{}
% \renewcommand\thesubsection{\Alph{subsection}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Reproducibility Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item This paper:
\begin{enumerate}
  \item Includes a conceptual outline and/or pseudocode description of AI methods introduced (\underline{yes}/partial/no/NA)
  \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (\underline{yes}/no)
  \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper (\underline{yes}/no)
\end{enumerate}

\item Does this paper make theoretical contributions? (yes/\underline{no})

\item Does this paper rely on one or more datasets? (\underline{yes}/no)
\begin{enumerate}
  \item A motivation is given for why the experiments are conducted on the selected datasets (\underline{yes}/partial/no/NA)
  \item All novel datasets introduced in this paper are included in a data appendix. (yes/partial/no/\underline{NA})
  \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no/\underline{NA})
  \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (\underline{yes}/no/NA)
  \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (\underline{yes}/partial/no/NA)
  \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisfying. (yes/partial/no/\underline{NA})
\end{enumerate}

\item Does this paper include computational experiments? (\underline{yes}/no)
\begin{enumerate}
  \item Any code required for pre-processing data is included in the appendix. (\underline{yes}/partial/no).
  \item All source code required for conducting and analyzing the experiments is included in a code appendix. (\underline{yes}/partial/no)
  \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (\underline{yes}/partial/no)
  \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (\underline{yes}/partial/no)
  \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes/partial/no/\underline{NA})
  \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (\underline{yes}/partial/no)
  \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (\underline{yes}/partial/no)
  \item This paper states the number of algorithm runs used to compute each reported result. (\underline{yes}/no)
  \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (\underline{yes}/no)
  \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes/partial/\underline{no})
  \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (\underline{yes}/partial/no/NA)
  \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (\underline{yes}/partial/no/NA)
\end{enumerate}

\end{enumerate}

==> sec_ours/checklist.tex <==
% \clearpage
% \setcounter{page}{1}
% \maketitlesupplementary

% \renewcommand\thesection{}
% \renewcommand\thesubsection{\Alph{subsection}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Reproducibility Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item This paper:
\begin{enumerate}
  \item Includes a conceptual outline and/or pseudocode description of AI methods introduced (\underline{yes}/partial/no/NA)
  \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (\underline{yes}/no)
  \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper (\underline{yes}/no)
\end{enumerate}

\item Does this paper make theoretical contributions? (yes/\underline{no})

\item Does this paper rely on one or more datasets? (\underline{yes}/no)
\begin{enumerate}
  \item A motivation is given for why the experiments are conducted on the selected datasets (\underline{yes}/partial/no/NA)
  \item All novel datasets introduced in this paper are included in a data appendix. (yes/partial/no/\underline{NA})
  \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no/\underline{NA})
  \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (\underline{yes}/no/NA)
  \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (\underline{yes}/partial/no/NA)
  \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisfying. (yes/partial/no/\underline{NA})
\end{enumerate}

\item Does this paper include computational experiments? (\underline{yes}/no)
\begin{enumerate}
  \item Any code required for pre-processing data is included in the appendix. (\underline{yes}/partial/no).
  \item All source code required for conducting and analyzing the experiments is included in a code appendix. (\underline{yes}/partial/no)
  \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (\underline{yes}/partial/no)
  \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (\underline{yes}/partial/no)
  \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes/partial/no/\underline{NA})
  \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (\underline{yes}/partial/no)
  \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (\underline{yes}/partial/no)
  \item This paper states the number of algorithm runs used to compute each reported result. (\underline{yes}/no)
  \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (\underline{yes}/no)
  \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes/partial/\underline{no})
  \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (\underline{yes}/partial/no/NA)
  \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (\underline{yes}/partial/no/NA)
\end{enumerate}

\end{enumerate}

==> tabs/tab_one.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\centering
% \resizebox{\textwidth}{75mm}{
\resizebox{1.8\columnwidth}{!}{%
\begin{tabular}{cccccccc}
\toprule[1.2pt]
\multirow{2}{*}{Evaluations}                                                                  & \multirow{2}{*}{Methods} & \multirow{2}{*}{VLMs} & \multicolumn{4}{c}{Datasets}                             & \multirow{2}{*}{Avg.}  \\ \cline{4-7}
                                                                                              &                          &                       & ImageNet-1K & CalTech-101 & Stanford-Dogs & CUB-200-2011 &                        \\ \toprule[1.0pt]
\multirow{16}{*}{\begin{tabular}[c]{@{}c@{}}Prediction \\ Accuracy (\%) ↑\end{tabular}} & \multirow{4}{*}{ZS}      & ALBEF-ViT-B/16        & 46.48       & 77.02       & 29.25         & 12.43        & \multirow{4}{*}{53.74} \\
                                                                                        &                          & BLIP-ViT-B/16         & 46.30       & 85.89       & 32.38         & 16.88        &                        \\
                                                                                        &                          & CLIP-ViT-B/16         & 63.30       & 84.22       & 60.61         & 54.94        &                        \\
                                                                                        &                          & CLIP-ViT-B/32         & 58.41       & 84.79       & 54.62         & 52.33        &                        \\ \cline{2-8} 
                                                                                        & \multirow{4}{*}{LP}      & ALBEF-ViT-B/16        & 72.03       & 90.38       & 65.10         & 48.46        & \multirow{4}{*}{72.50} \\
                                                                                        &                          & BLIP-ViT-B/16         & 72.46       & 90.26       & 64.23         & 47.77        &                        \\
                                                                                        &                          & CLIP-ViT-B/16         & 76.69       & 94.64       & 74.14         & 70.14        &                        \\
                                                                                        &                          & CLIP-ViT-B/32         & 72.21       & 93.09       & 67.27         & 61.08        &                        \\ \cline{2-8} 
                                                                                        & \multirow{4}{*}{FLCP}    & ALBEF-ViT-B/16        & 77.58       & 95.85       & 77.88         & 77.27        & \multirow{4}{*}{\underline{80.99}} \\
                                                                                        &                          & BLIP-ViT-B/16         & 78.67       & 94.99       & 77.89         & 68.85        &                        \\
                                                                                        &                          & CLIP-ViT-B/16         & 72.41       & 96.20       & 80.70         & 80.76        &                        \\
                                                                                        &                          & CLIP-ViT-B/32         & 70.81       & 95.74       & 75.70         & 74.49        &                        \\ \cline{2-8} 
                                                                                        & \multirow{4}{*}{FT}      & ALBEF-ViT-B/16        & 80.82       & 95.91       & 81.32         & 80.48        & \multirow{4}{*}{\textbf{81.63}} \\
                                                                                        &                          & BLIP-ViT-B/16         & 80.75       & 92.74       & 78.68         & 68.98        &                        \\
                                                                                        &                          & CLIP-ViT-B/16         & 81.19       & 93.03       & 81.56         & 79.25        &                        \\
                                                                                        &                          & CLIP-ViT-B/32         & 76.62       & 94.30       & 72.42         & 68.07        &                        \\ \toprule[0.75pt]
\multirow{16}{*}{\begin{tabular}[c]{@{}c@{}}Prediction\\ Trustworthiness\\ (PT, \%) ↑\end{tabular}} & \multirow{4}{*}{ZS}      & ALBEF-ViT-B/16        & 90.61       & 76.28       & 95.02         & 49.31        & \multirow{4}{*}{\textbf{71.26}} \\
                                                                                              &                          & BLIP-ViT-B/16         & 89.01       & 61.72       & 93.95         & 23.93        &                        \\
                                                                                              &                          & CLIP-ViT-B/16         & 87.05       & 62.99       & 92.96         & 29.38        &                        \\
                                                                                              &                          & CLIP-ViT-B/32         & 89.39       & 73.44       & 94.58         & 30.57        &                        \\ \cline{2-8} 
                                                                                              & \multirow{4}{*}{LP}      & ALBEF-ViT-B/16        & 82.37       & 59.08       & 90.30         & 19.91        & \multirow{4}{*}{64.78} \\
                                                                                              &                          & BLIP-ViT-B/16         & 80.36       & 52.57       & 92.63         & 12.98        &                        \\
                                                                                              &                          & CLIP-ViT-B/16         & 80.65       & 56.40       & 92.19         & 36.17        &                        \\
                                                                                              &                          & CLIP-ViT-B/32         & 84.05       & 68.22       & 92.76         & 35.89        &                        \\ \cline{2-8} 
                                                                                              & \multirow{4}{*}{FLCP}    & ALBEF-ViT-B/16        & 87.07       & 62.43       & 92.68         & 64.33        & \multirow{4}{*}{\underline{67.95}} \\
                                                                                              &                          & BLIP-ViT-B/16         & 82.57       & 59.52       & 91.46         & 36.17        &                        \\
                                                                                              &                          & CLIP-ViT-B/16         & 81.40       & 64.32       & 76.44         & 16.56        &                        \\
                                                                                              &                          & CLIP-ViT-B/32         & 85.48       & 71.29       & 91.59         & 23.84        &                        \\ \cline{2-8} 
                                                                                              & \multirow{4}{*}{FT}      & ALBEF-ViT-B/16        & 86.28       & 48.97       & 92.22         & 24.98        & \multirow{4}{*}{67.01} \\
                                                                                              &                          & BLIP-ViT-B/16         & 85.54       & 39.96       & 93.13         & 25.85        &                        \\
                                                                                              &                          & CLIP-ViT-B/16         & 82.98       & 56.86       & 91.60         & 27.98        &                        \\
                                                                                              &                          & CLIP-ViT-B/32         & 86.29       & 80.01       & 94.17         & 55.43        &                        \\ \toprule[0.75pt]
\multirow{16}{*}{\begin{tabular}[c]{@{}c@{}}Inference\\ Reliability\\ (IR, \%) ↑\end{tabular}}      & \multirow{4}{*}{ZS}      & ALBEF-ViT-B/16        & 48.95       & 76.74       & 30.56         & 16.43        & \multirow{4}{*}{56.65} \\
                                                                                              &                          & BLIP-ViT-B/16         & 49.65       & 90.05       & 33.87         & 18.92        &                        \\
                                                                                              &                          & CLIP-ViT-B/16         & 66.33       & 85.58       & 61.96         & 68.05        &                        \\
                                                                                              &                          & CLIP-ViT-B/32         & 61.09       & 85.23       & 56.12         & 56.80        &                        \\ \cline{2-8} 
                                                                                              & \multirow{4}{*}{LP}      & ALBEF-ViT-B/16        & 74.76       & 92.56       & 66.21         & 55.46        & \multirow{4}{*}{75.67} \\
                                                                                              &                          & BLIP-ViT-B/16         & 74.78       & 90.89       & 65.11         & 59.91        &                        \\
                                                                                              &                          & CLIP-ViT-B/16         & 78.93       & 95.05       & 75.41         & 77.08        &                        \\
                                                                                              &                          & CLIP-ViT-B/32         & 74.91       & 93.76       & 68.53         & 67.37        &                        \\ \cline{2-8} 
                                                                                              & \multirow{4}{*}{FLCP}    & ALBEF-ViT-B/16        & 78.54       & 96.81       & 78.36         & 80.92        & \multirow{4}{*}{\underline{81.71}} \\
                                                                                              &                          & BLIP-ViT-B/16         & 80.04       & 94.93       & 78.73         & 73.40        &                        \\
                                                                                              &                          & CLIP-ViT-B/16         & 75.00       & 94.84       & 80.21         & 77.97        &                        \\
                                                                                              &                          & CLIP-ViT-B/32         & 71.84       & 95.46       & 76.43         & 73.87        &                        \\ \cline{2-8} 
                                                                                              & \multirow{4}{*}{FT}      & ALBEF-ViT-B/16        & 82.95       & 94.41       & 81.93         & 81.87        & \multirow{4}{*}{\textbf{83.52}} \\
                                                                                              &                          & BLIP-ViT-B/16         & 82.86       & 91.55       & 79.18         & 85.26        &                        \\
                                                                                              &                          & CLIP-ViT-B/16         & 83.25       & 90.66       & 82.06         & 81.12        &                        \\
                                                                                              &                          & CLIP-ViT-B/32         & 79.34       & 93.86       & 73.22         & 72.72        &                        \\ \bottomrule[1.2pt]
\end{tabular}
}
\caption{Comparisons of four methods with proposed ``PT'' and ``IR'' metrics. Here we observe that mainstream fine-tuning methods come with both strengths and weaknesses. We show that fine-tuning mostly leads to a worse capability of prediction trustworthiness but enhances the inference reliability of VLMs than the ZS method. The best-averaged score among the four methods is \textbf{bolded}, while the second-place averaged score among the four methods is \underline{underlined}.}
\label{tab_ptir}
\end{table*}

==> tabs/tab_pt_ir_3.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[h]
\centering
% \resizebox{\textwidth}{65mm}{
\resizebox{1.8\columnwidth}{!}{%
\begin{tabular}{cccccccc}
\toprule[1.2pt]
\multirow{2}{*}{Evaluations}                                                                  & \multirow{2}{*}{Methods} & \multirow{2}{*}{VLMs} & \multicolumn{4}{c}{Datasets}                             & \multirow{2}{*}{Avg.}  \\ \cline{4-7}
                                                                                              &                          &                       & ImageNet-1K & CalTech-101 & Stanford-Dogs & CUB-200-2011 &                        \\ \toprule[1.0pt]
\multirow{20}{*}{\begin{tabular}[c]{@{}c@{}}Prediction\\ Trustworthiness\\ (PT, \%) ↑\end{tabular}} & \multirow{4}{*}{ZS}      & ALBEF-ViT-B/16        & 90.61       & 76.28       & 95.02         & 49.31        & \multirow{4}{*}{\textbf{71.26}} \\
                                                                                              &                          & BLIP-ViT-B/16         & 89.01       & 61.72       & 93.95         & 23.93        &                        \\
                                                                                              &                          & CLIP-ViT-B/16         & 87.05       & 62.99       & 92.96         & 29.38        &                        \\
                                                                                              &                          & CLIP-ViT-B/32         & 89.39       & 73.44       & 94.58         & 30.57        &                        \\ \cline{2-8} 
                                                                                              & \multirow{4}{*}{LP}      & ALBEF-ViT-B/16        & 82.37       & 59.08       & 90.30         & 19.91        & \multirow{4}{*}{64.78} \\
                                                                                              &                          & BLIP-ViT-B/16         & 80.36       & 52.57       & 92.63         & 12.98        &                        \\
                                                                                              &                          & CLIP-ViT-B/16         & 80.65       & 56.40       & 92.19         & 36.17        &                        \\
                                                                                              &                          & CLIP-ViT-B/32         & 84.05       & 68.22       & 92.76         & 35.89        &                        \\ \cline{2-8} 
                                                                                              & \multirow{4}{*}{FLCP}    & ALBEF-ViT-B/16        & 87.07       & 62.43       & 92.68         & 64.33        & \multirow{4}{*}{\underline{67.95}} \\
                                                                                              &                          & BLIP-ViT-B/16         & 82.57       & 59.52       & 91.46         & 36.17        &                        \\
                                                                                              &                          & CLIP-ViT-B/16         & 81.40       & 64.32       & 76.44         & 16.56        &                        \\
                                                                                              &                          & CLIP-ViT-B/32         & 85.48       & 71.29       & 91.59         & 23.84        &                        \\ \cline{2-8} 
                                                                                              & \multirow{4}{*}{FT}      & ALBEF-ViT-B/16        & 86.28       & 48.97       & 92.22         & 24.98        & \multirow{4}{*}{67.01} \\
                                                                                              &                          & BLIP-ViT-B/16         & 85.54       & 39.96       & 93.13         & 25.85        &                        \\
                                                                                              &                          & CLIP-ViT-B/16         & 82.98       & 56.86       & 91.60         & 27.98        &                        \\
                                                                                              &                          & CLIP-ViT-B/32         & 86.29       & 80.01       & 94.17         & 55.43        &                        \\ \cline{2-8} 
                                                                                              & \multirow{4}{*}{CoOp}      & ALBEF-ViT-B/16        & 00.00       & 00.00       & 00.00         & 00.00        & \multirow{4}{*}{00.00} \\
                                                                                              &                          & BLIP-ViT-B/16         & 00.00       & 00.00       & 00.00         & 00.00        &                        \\
                                                                                              &                          & CLIP-ViT-B/16         & 00.00       & 35.94       & 00.00         & 00.00        &                        \\
                                                                                              &                          & CLIP-ViT-B/32         & 00.00       & 47.96       & 00.00         & 00.00        &                        \\ \toprule[0.75pt]
\multirow{20}{*}{\begin{tabular}[c]{@{}c@{}}Inference\\ Reliability\\ (IR, \%) ↑\end{tabular}}      & \multirow{4}{*}{ZS}      & ALBEF-ViT-B/16        & 48.95       & 76.74       & 30.56         & 16.43        & \multirow{4}{*}{56.65} \\
                                                                                              &                          & BLIP-ViT-B/16         & 49.65       & 90.05       & 33.87         & 18.92        &                        \\
                                                                                              &                          & CLIP-ViT-B/16         & 66.33       & 85.58       & 61.96         & 68.05        &                        \\
                                                                                              &                          & CLIP-ViT-B/32         & 61.09       & 85.23       & 56.12         & 56.80        &                        \\ \cline{2-8} 
                                                                                              & \multirow{4}{*}{LP}      & ALBEF-ViT-B/16        & 74.76       & 92.56       & 66.21         & 55.46        & \multirow{4}{*}{75.67} \\
                                                                                              &                          & BLIP-ViT-B/16         & 74.78       & 90.89       & 65.11         & 59.91        &                        \\
                                                                                              &                          & CLIP-ViT-B/16         & 78.93       & 95.05       & 75.41         & 77.08        &                        \\
                                                                                              &                          & CLIP-ViT-B/32         & 74.91       & 93.76       & 68.53         & 67.37        &                        \\ \cline{2-8} 
                                                                                              & \multirow{4}{*}{FLCP}    & ALBEF-ViT-B/16        & 78.54       & 96.81       & 78.36         & 80.92        & \multirow{4}{*}{\underline{81.71}} \\
                                                                                              &                          & BLIP-ViT-B/16         & 80.04       & 94.93       & 78.73         & 73.40        &                        \\
                                                                                              &                          & CLIP-ViT-B/16         & 75.00       & 94.84       & 80.21         & 77.97        &                        \\
                                                                                              &                          & CLIP-ViT-B/32         & 71.84       & 95.46       & 76.43         & 73.87        &                        \\ \cline{2-8} 
                                                                                              & \multirow{4}{*}{FT}      & ALBEF-ViT-B/16        & 82.95       & 94.41       & 81.93         & 81.87        & \multirow{4}{*}{\textbf{83.52}} \\
                                                                                              &                          & BLIP-ViT-B/16         & 82.86       & 91.55       & 79.18         & 85.26        &                        \\
                                                                                              &                          & CLIP-ViT-B/16         & 83.25       & 90.66       & 82.06         & 81.12        &                        \\
                                                                                              &                          & CLIP-ViT-B/32         & 79.34       & 93.86       & 73.22         & 72.72        &                        \\ \cline{2-8} 
                                                                                            & \multirow{4}{*}{CoOp}      & ALBEF-ViT-B/16        & 00.00       & 00.00       & 00.00         & 00.00        & \multirow{4}{*}{00.00} \\
                                                                                              &                          & BLIP-ViT-B/16         & 00.00       & 00.00       & 00.00         & 00.00        &                        \\
                                                                                              &                          & CLIP-ViT-B/16         & 00.00       & 96.13       & 00.00         & 00.00        &                        \\
                                                                                              &                          & CLIP-ViT-B/32         & 00.00       & 92.82       & 00.00         & 00.00        &                        \\ \bottomrule[1.2pt]
\end{tabular}
}
\caption{Comparisons of four methods with proposed ``PT'' (\ref{formula_pt}) and ``IR'' (\ref{formula_ir}) metrics. Here we observe that mainstream fine-tuning methods come with both strengths and weaknesses. We show that fine-tuning mostly leads to a worse capability of prediction trustworthiness but enhances the inference reliability of VLMs than the ZS method. The best-averaged score among the four methods is \textbf{bolded}, while the second-place averaged score among the four methods is \underline{underlined}.}
\label{tab_ptir}
\end{table*}

==> tabs/tab_what_2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\centering
% \resizebox{\textwidth}{65mm}{
\resizebox{2.0\columnwidth}{!}{%
\begin{tabular}{cccccccc}
\toprule[1.2pt]
\multirow{2}{*}{Evaluations}                                                            & \multirow{2}{*}{Methods} & \multirow{2}{*}{VLMs} & \multicolumn{4}{c}{Datasets}                             & \multirow{2}{*}{Avg.}  \\ \cline{4-7}
                                                                                        &                          &                       & ImageNet-1K & CalTech-101 & Stanford-Dogs & CUB-200-2011 &                        \\ \bottomrule[1.0pt]
\multirow{16}{*}{\begin{tabular}[c]{@{}c@{}}Prediction \\ Accuracy (\%) ↑\end{tabular}} & \multirow{4}{*}{ZS}      & ALBEF-ViT-B/16        & 46.48       & 77.02       & 29.25         & 12.43        & \multirow{4}{*}{53.74} \\
                                                                                        &                          & BLIP-ViT-B/16         & 46.30       & 85.89       & 32.38         & 16.88        &                        \\
                                                                                        &                          & CLIP-ViT-B/16         & 63.30       & 84.22       & 60.61         & 54.94        &                        \\
                                                                                        &                          & CLIP-ViT-B/32         & 58.41       & 84.79       & 54.62         & 52.33        &                        \\ \cline{2-8} 
                                                                                        & \multirow{4}{*}{LP}      & ALBEF-ViT-B/16        & 72.03       & 90.38       & 65.10         & 48.46        & \multirow{4}{*}{72.50} \\
                                                                                        &                          & BLIP-ViT-B/16         & 72.46       & 90.26       & 64.23         & 47.77        &                        \\
                                                                                        &                          & CLIP-ViT-B/16         & 76.69       & 94.64       & 74.14         & 70.14        &                        \\
                                                                                        &                          & CLIP-ViT-B/32         & 72.21       & 93.09       & 67.27         & 61.08        &                        \\ \cline{2-8} 
                                                                                        & \multirow{4}{*}{FLCP}    & ALBEF-ViT-B/16        & 77.58       & 95.85       & 77.88         & 77.27        & \multirow{4}{*}{\underline{80.99}} \\
                                                                                        &                          & BLIP-ViT-B/16         & 78.67       & 94.99       & 77.89         & 68.85        &                        \\
                                                                                        &                          & CLIP-ViT-B/16         & 72.41       & 96.20       & 80.70         & 80.76        &                        \\
                                                                                        &                          & CLIP-ViT-B/32         & 70.81       & 95.74       & 75.70         & 74.49        &                        \\ \cline{2-8} 
                                                                                        & \multirow{4}{*}{FT}      & ALBEF-ViT-B/16        & 80.82       & 95.91       & 81.32         & 80.48        & \multirow{4}{*}{\textbf{81.63}} \\
                                                                                        &                          & BLIP-ViT-B/16         & 80.75       & 92.74       & 78.68         & 68.98        &                        \\
                                                                                        &                          & CLIP-ViT-B/16         & 81.19       & 93.03       & 81.56         & 79.25        &                        \\
                                                                                        &                          & CLIP-ViT-B/32         & 76.62       & 94.30       & 72.42         & 68.07        &                        \\ \toprule[0.75pt]
\multirow{16}{*}{\begin{tabular}[c]{@{}c@{}} RMA (\%) ↑\end{tabular}}   & \multirow{4}{*}{ZS}      & ALBEF-ViT-B/16        & 80.22       & 61.55       & 86.03         & 47.78        & \multirow{4}{*}{\textbf{65.65}} \\
                                                                                        &                          & BLIP-ViT-B/16         & 77.17       & 55.02       & 80.90         & 40.18        &                        \\
                                                                                        &                          & CLIP-ViT-B/16         & 76.86       & 55.44       & 83.04         & 40.81        &                        \\
                                                                                        &                          & CLIP-ViT-B/32         & 79.40       & 60.19       & 85.01         & 40.80        &                        \\ \cline{2-8} 
                                                                                        & \multirow{4}{*}{LP}      & ALBEF-ViT-B/16        & 72.21       & 52.93       & 75.99         & 39.04        & \multirow{4}{*}{61.37} \\
                                                                                        &                          & BLIP-ViT-B/16         & 71.20       & 51.59       & 78.61         & 37.25        &                        \\
                                                                                        &                          & CLIP-ViT-B/16         & 71.34       & 52.91       & 78.65         & 44.26        &                        \\
                                                                                        &                          & CLIP-ViT-B/32         & 74.22       & 57.16       & 81.00         & 43.55        &                        \\ \cline{2-8} 
                                                                                        & \multirow{4}{*}{FLCP}    & ALBEF-ViT-B/16        & 78.04       & 53.54       & 82.95         & 52.99        & \multirow{4}{*}{62.06} \\
                                                                                        &                          & BLIP-ViT-B/16         & 73.09       & 52.86       & 80.28         & 42.96        &                        \\
                                                                                        &                          & CLIP-ViT-B/16         & 69.70       & 53.27       & 68.06         & 32.45        &                        \\
                                                                                        &                          & CLIP-ViT-B/32         & 76.62       & 59.47       & 80.33         & 36.42        &                        \\ \cline{2-8} 
                                                                                        & \multirow{4}{*}{FT}      & ALBEF-ViT-B/16        & 74.57       & 50.01       & 77.25         & 41.84        & \multirow{4}{*}{\underline{62.40}} \\
                                                                                        &                          & BLIP-ViT-B/16         & 73.33       & 46.47       & 77.85         & 42.27        &                        \\
                                                                                        &                          & CLIP-ViT-B/16         & 72.12       & 52.67       & 75.76         & 42.93        &                        \\
                                                                                        &                          & CLIP-ViT-B/32         & 76.14       & 61.88       & 83.60         & 49.72        &                        \\ \bottomrule[1.2pt]
\end{tabular}
}
\caption{Comparisons of four methods regarding prediction accuracy and RMA. We find fine-tuning mostly leads VLMs to provide invalid evidence when making predictions, despite improving prediction capability than the zero-shot (ZS) method. The best-averaged score among the four methods is \textbf{bolded}, while the second-place averaged score is \underline{underlined}. RMA is evaluated for data samples with correct predictions. }
\label{tab_what}
\end{table*}

==> tabs/tab_what_3.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\centering
% \resizebox{\textwidth}{70mm}{
\resizebox{1.8\columnwidth}{!}{%
\begin{tabular}{cccccccc}
\toprule[1.2pt]
\multirow{2}{*}{Evaluations}                                                            & \multirow{2}{*}{Methods} & \multirow{2}{*}{VLMs} & \multicolumn{4}{c}{Datasets}                             & \multirow{2}{*}{Avg.}  \\ \cline{4-7}
                                                                                        &                          &                       & ImageNet-1K & CalTech-101 & Stanford-Dogs & CUB-200-2011 &                        \\ \bottomrule[1.0pt]
\multirow{20}{*}{\begin{tabular}[c]{@{}c@{}}Prediction \\ Accuracy (\%) ↑\end{tabular}} & \multirow{4}{*}{ZS}      & ALBEF-ViT-B/16        & 46.48       & 77.02       & 29.25         & 12.43        & \multirow{4}{*}{53.74} \\
                                                                                        &                          & BLIP-ViT-B/16         & 46.30       & 85.89       & 32.38         & 16.88        &                        \\
                                                                                        &                          & CLIP-ViT-B/16         & 63.30       & 84.22       & 60.61         & 54.94        &                        \\
                                                                                        &                          & CLIP-ViT-B/32         & 58.41       & 84.79       & 54.62         & 52.33        &                        \\ \cline{2-8} 
                                                                                        & \multirow{4}{*}{LP}      & ALBEF-ViT-B/16        & 72.03       & 90.38       & 65.10         & 48.46        & \multirow{4}{*}{72.50} \\
                                                                                        &                          & BLIP-ViT-B/16         & 72.46       & 90.26       & 64.23         & 47.77        &                        \\
                                                                                        &                          & CLIP-ViT-B/16         & 76.69       & 94.64       & 74.14         & 70.14        &                        \\
                                                                                        &                          & CLIP-ViT-B/32         & 72.21       & 93.09       & 67.27         & 61.08        &                        \\ \cline{2-8} 
                                                                                        & \multirow{4}{*}{FLCP}    & ALBEF-ViT-B/16        & 77.58       & 95.85       & 77.88         & 77.27        & \multirow{4}{*}{\underline{80.99}} \\
                                                                                        &                          & BLIP-ViT-B/16         & 78.67       & 94.99       & 77.89         & 68.85        &                        \\
                                                                                        &                          & CLIP-ViT-B/16         & 72.41       & 96.20       & 80.70         & 80.76        &                        \\
                                                                                        &                          & CLIP-ViT-B/32         & 70.81       & 95.74       & 75.70         & 74.49        &                        \\ \cline{2-8} 
                                                                                        & \multirow{4}{*}{FT}      & ALBEF-ViT-B/16        & 80.82       & 95.91       & 81.32         & 80.48        & \multirow{4}{*}{\textbf{81.63}} \\
                                                                                        &                          & BLIP-ViT-B/16         & 80.75       & 92.74       & 78.68         & 68.98        &                        \\
                                                                                        &                          & CLIP-ViT-B/16         & 81.19       & 93.03       & 81.56         & 79.25        &                        \\
                                                                                        &                          & CLIP-ViT-B/32         & 76.62       & 94.30       & 72.42         & 68.07        &                        \\ \cline{2-8} 
                                                                                        & \multirow{4}{*}{CoOp}      & ALBEF-ViT-B/16        & 00.00       & 00.00       & 00.00         & 00.00        & \multirow{4}{*}{00.00} \\
                                                                                        &                          & BLIP-ViT-B/16         & 00.00       & 00.00       & 00.00         & 00.00        &                        \\
                                                                                        &                          & CLIP-ViT-B/16         & 00.00       & 92.17       & 00.00         & 00.00        &                        \\
                                                                                        &                          & CLIP-ViT-B/32         & 00.00       & 92.28       & 00.00         & 00.00        &                        \\ \toprule[0.75pt]
\multirow{20}{*}{\begin{tabular}[c]{@{}c@{}}Explainability  \\ RMA (\%) ↑\end{tabular}}   & \multirow{4}{*}{ZS}      & ALBEF-ViT-B/16        & 80.22       & 61.55       & 86.03         & 47.78        & \multirow{4}{*}{\textbf{65.65}} \\
                                                                                        &                          & BLIP-ViT-B/16         & 77.17       & 55.02       & 80.90         & 40.18        &                        \\
                                                                                        &                          & CLIP-ViT-B/16         & 76.86       & 55.44       & 83.04         & 40.81        &                        \\
                                                                                        &                          & CLIP-ViT-B/32         & 79.40       & 60.19       & 85.01         & 40.80        &                        \\ \cline{2-8} 
                                                                                        & \multirow{4}{*}{LP}      & ALBEF-ViT-B/16        & 72.21       & 52.93       & 75.99         & 39.04        & \multirow{4}{*}{61.37} \\
                                                                                        &                          & BLIP-ViT-B/16         & 71.20       & 51.59       & 78.61         & 37.25        &                        \\
                                                                                        &                          & CLIP-ViT-B/16         & 71.34       & 52.91       & 78.65         & 44.26        &                        \\
                                                                                        &                          & CLIP-ViT-B/32         & 74.22       & 57.16       & 81.00         & 43.55        &                        \\ \cline{2-8} 
                                                                                        & \multirow{4}{*}{FLCP}    & ALBEF-ViT-B/16        & 78.04       & 53.54       & 82.95         & 52.99        & \multirow{4}{*}{62.06} \\
                                                                                        &                          & BLIP-ViT-B/16         & 73.09       & 52.86       & 80.28         & 42.96        &                        \\
                                                                                        &                          & CLIP-ViT-B/16         & 69.70       & 53.27       & 68.06         & 32.45        &                        \\
                                                                                        &                          & CLIP-ViT-B/32         & 76.62       & 59.47       & 80.33         & 36.42        &                        \\ \cline{2-8} 
                                                                                        & \multirow{4}{*}{FT}      & ALBEF-ViT-B/16        & 74.57       & 50.01       & 77.25         & 41.84        & \multirow{4}{*}{\underline{62.40}} \\
                                                                                        &                          & BLIP-ViT-B/16         & 73.33       & 46.47       & 77.85         & 42.27        &                        \\
                                                                                        &                          & CLIP-ViT-B/16         & 72.12       & 52.67       & 75.76         & 42.93        &                        \\
                                                                                        &                          & CLIP-ViT-B/32         & 76.14       & 61.88       & 83.60         & 49.72        &                        \\ \cline{2-8} 
                                                                                        & \multirow{4}{*}{CoOp}      & ALBEF-ViT-B/16        & 00.00       & 00.00       & 00.00         & 00.00        & \multirow{4}{*}{00.00} \\
                                                                                        &                          & BLIP-ViT-B/16         & 00.00       & 00.00       & 00.00         & 00.00        &                        \\
                                                                                        &                          & CLIP-ViT-B/16         & 00.00       & 46.31       & 00.00         & 00.00        &                        \\
                                                                                        &                          & CLIP-ViT-B/32         & 00.00       & 50.02       & 00.00         & 00.00        &                        \\ \bottomrule[1.2pt]
\end{tabular}
}
\caption{Comparisons of four methods regarding prediction and explanation accuracy. We find fine-tuning mostly leads to worse explanation accuracies despite improving prediction capability than the zero-shot (ZS) method. The best-averaged score among the four methods is \textbf{bolded}, while the second-place averaged score is \underline{underlined}. Explanation accuracy is evaluated for data samples with correct predictions. }
\label{tab_what}
\end{table*}
